Pathologies of Predictive Diversity in Deep Ensembles

Classic results establish that encouraging predictive diversity improves performance in ensembles of low-capacity models, e.g. through bagging or boosting. Here we demonstrate that these intuitions do not apply to high-capacity neural network ensembles (deep ensembles), and in fact the opposite is often true. In a large scale study of nearly 600 neural network classification ensembles, we examine a variety of interventions that trade off component model performance for predictive diversity. While such interventions can improve the performance of small neural network ensembles (in line with standard intuitions), they harm the performance of the large neural network ensembles most often used in practice. Surprisingly, we also find that discouraging predictive diversity is often benign in large-network ensembles, fully inverting standard intuitions. Even when diversity-promoting interventions do not sacrifice component model performance (e.g. using heterogeneous architectures and training paradigms), we observe an opportunity cost associated with pursuing increased predictive diversity. Examining over 1000 ensembles, we observe that the performance benefits of diverse architectures/training procedures are easily dwarfed by the benefits of simply using higher-capacity models, despite the fact that such higher capacity models often yield significantly less predictive diversity. Overall, our findings demonstrate that standard intuitions around predictive diversity, originally developed for low-capacity ensembles, do not directly apply to modern high-capacity deep ensembles. This work clarifies fundamental challenges to the goal of improving deep ensembles by making them more diverse, while suggesting an alternative path: simply forming ensembles from ever more powerful (and less diverse) component models.

==> sections/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

The results in the previous section
empirically demonstrate that encouraging predictive diversity---%
while beneficial for regression and small-model classification---%
is detrimental for large-model classification.
In \cref{sec:intuition}, we presented two observations about large-scale classification models that could generate this discrepancy.
In this section, we offer empirical evidence to confirm these observations.


\begin{figure*}
    \centering
    \subfloat{\includegraphics[width=0.59\textwidth]{figs/counterfactual_accuracy_vs_diversity_cifar10_resnet18.pdf}}
    \subfloat{\includegraphics[width=0.3\linewidth]{figs/schematic.pdf}}
    \vspace{-0.9em}
    \caption{
        {\bf Left: Regularization increases the diversity of all predictions,
        not just errors.}
        (\textbf{Top}) histograms of per-datapoint predictive diversity (as measured by the cross-entropy Jensen gap) for ensembles with various regularizers.
        (\textbf{Bottom}) dividing all predictions into bins based on their predictive diversity, we compute the per-bin \emph{counterfactual ensemble accuracy}---the likelihood that an ensemble would have made a correct prediction  absent regularization for datapoints in a given bin.
        (Bins are smoothed with a Gaussian kernel.)
        (\textbf{Main takeaway}) while regularization increases predictive diversity on a per-datapoint level,
        regularized predictions with high diversity are counterfactually more likely to have been correct.
        \textbf{Right: Regardless of encouragement strategy, diversity is impossible at extreme points.} Under 3 different methods of adding diversity to a perfect ensemble prediction (geometric scaling, sampling in logit space, or sampling from a dirichlet distribution), \textit{any} of these strategies will degrade average single model loss more rapidly than increases in predictive diversity, leading to worse ensemble performance overall. 
    }
    \label{fig:counterfactual_accuracy_cifar10_resnet18}
    \vspace{-1em}
\end{figure*}

\textbf{Observation 1: Diversity encouragement impacts all ensemble predictions, not only the incorrect ones.} 
Ideally, diversity-encouraging regularizers would only decorrelate what would otherwise be erroneous predictions, without modifying correct predictions.
However, as suggested in \cref{sec:intuition}, it is more likely that diversity regularizers affect all predictions---whether erroneous or correct.
To test this hypothesis for a given ensemble, we bin all datapoints based on their predictive diversity,
and then we consider the \emph{counterfactual ensemble accuracy} of datapoints in each bin---%
i.e. whether a given ensemble with any amount of regularization would have made the correct prediction absent that regularization.
We perform this analysis for ResNet-18 CIFAR10 ensembles trained with diversity encouragement.
\cref{fig:counterfactual_accuracy_cifar10_resnet18} plots histograms of each diversity bin (top row) as well as the counterfactual accuracy of each diversity bin (bottom row), where all plots are smoothed with a Gaussian kernel.

From these plots we can observe numerous trends that hold across all regularizers.
Without any diversity-encouraging regularization (black curves, $\gamma = 0$)  a majority of predictions incur little diversity (CE Jensen Gap $< 0.1$), and counterfactual predictive accuracy decays slowly as a function of (per-datapoint) predictive diversity. 
If diversity encouragement only decorrelated errors, we would expect this relationship to sharpen: \textit{higher} values of counterfactual ensemble accuracy at low values of predictive diversity, and \textit{lower} values on data that expresses more diversity. 
Instead, as we apply diversity-encouraging regularizers ($\gamma < 0$), we observe that a \textit{greater} portion of diverse predictions are counterfactually correct, implying that most datapoints with increased diversity were classified correctly to begin with.  
As a dramatic example, with a $\gamma\!=\!-9$ variance-regularized ensemble, most predictions yield a CE Jensen Gap of $\approx 0.5$.
However, $95\%$ of the data with this amount predictive diversity would have been correctly classified without diversity interventions.
Indeed, for all regularized ensembles, the counterfactual accuracy around diversity mode is always around $94\%$, the overall (unconditional) accuracy of the unregularized ensemble.
These results demonstrate that the training interventions we study indiscriminately increase predictive diversity of all datapoints, regardless of whether these predictions would have have otherwise been correct.


\textbf{Observation 2: In constrained prediction spaces, diversity is impossible at extreme points.}
Finally, we demonstrate that---for nearly perfect predictions---increasing diversity yields worse ensemble performance on a per-datapoint level. 
In \cref{fig:counterfactual_accuracy_cifar10_resnet18} (right), we plot how a single perfect ensemble prediction would respond to increased diversity across component models.
We consider three potential mechanisms that could result in increased diversity: a geometric scaling of predictions, drawing predictions from a simple distribution, or adding noise to the underlying set of prediction logits (see \cref{appx:toy} for details).
As predicted in \cref{sec:intuition}, all mechanisms result in a worse ensemble prediction (higher diagonal level sets) as the diversity across models is increased.
We also note that \cref{fig:counterfactual_accuracy_cifar10_resnet18} (right) also offers a plausible explanation for the anticorrelation between predictive diversity and ensemble performance in \cref{fig:all_indep_models}: better individual models (which yield better ensembles) are more likely to make predictions in the extreme points of the simplex \citep{guo2017calibration}. 

\textbf{Taken together,} these observations suggest why predictive diversity is only harmful for large-capacity classification ensembles.
We note that Observation 1 is only harmful in settings where Observation 2 applies.
Thus, while regression and low-capacity classification models are also subject to Observation 1 (indiscriminate predictive diversity increases), the effect is not inherently harmful since its predictions do not lie on boundary points.



==> sections/experiments.tex <==
\section{Manipulating predictive diversity in neural network ensembles}
\label{sec:experimental_setup}


To test our hypotheses,
we perform large-scale experiments measuring to what extent \emph{encouraging versus discouraging} predictive diversity affects deep ensemble performance.
In particular, we aim to compare and contrast the behavior of large-model classification deep ensembles (for which we expect diversity to be harmful) versus regression and small-model deep ensembles (for which we expect diversity to be helpful).
In total, we train 574 ensembles across two datasets and six architectures, using four regularizers that encourage/discourage ensemble diversity.

\begin{figure*}[!t]
\centering
\subfloat{\includegraphics[width=1.0\linewidth]{figs/all_weight_resnet18_cifar10.pdf}}
\vspace{-1em}
\caption{\textbf{Ensemble performance improves as we penalize predictive diversity}. We train diversity regularized deep ensembles using \cref{eqn:loss_gamma} on CIFAR10. Each column corresponds to a different regularizer in \cref{sec:measuring_diversity} applied to ResNet18 ensembles (for other architectures, CIFAR100, and TinyImageNet, see \cref{appx:replications}).  
We compare normal ensemble training loss (dotted line) to regularization that encourage predictive diversity (left of dotted line). For all regularizers we use to control predictive diversity (Jensen Gap, Variance, JSD 1 vs. All, JSD Average), test accuracy suffers with increasing diversity encouragement, dropping out of the range of standard ensemble performance (blue bands), and sometimes below that of single model performance (black bands), whereas diversity discouragement can be benign. 
}
\vspace{-1em}
\label{fig:diversity_plots}
\end{figure*}

\begin{figure*}[!t]
\centering
\includegraphics[width=1\linewidth]{figs/biasvar_cifar10.pdf}
\vspace{-2em}
\caption{
    \textbf{Measuring predictive diversity in diversity regularized ensembles.} 
    Each marker represents a ResNet18 ensemble from \cref{fig:diversity_plots} trained on CIFAR10 (see \cref{appx:replications} for CIFAR100).
     Warmer colors correspond to positive $\gamma$ values (encouraging predictive diversity), while the cooler colors correspond to negative $\gamma$ values (discouraging predictive diversity). 
    The level set of standard deep ensemble performance ($\gamma=0$) is denoted by $\times$ and
    the dotted diagonal line.
    Ensembles where diversity was encouraged ($\gamma<0$; blue markers) express more predictive diversity than standard ensembles, but at the cost of average single model performance. Corresponding ensemble performance is \textit{worse} (above dotted line) than standard ensembling, as measured by NLL. In contrast, discouraging predictive diversity ($\gamma>0$; red markers) generates ensembles that can outperform standard training (below the dotted line). The ensemble with the best test NLL is one where diversity was discouraged.
    }
\label{fig:biasvar_decomp}
\vspace{-1em}
\end{figure*}


\textbf{Methods.}
We consider four methods to encourage/discourage predictive diversity.
Each can be formulated as a regularized version of standard ensemble training (Eq.~\ref{eqn:ens_training_objective}):
%
\begin{equation}
    \begin{split}
        \mathcal{L}_\text{avg} - \E_{p(\!\vx, y\!)} \! \Bigl[ \!
        - \: \gamma \underbracket{\mathbb{D}\!\left(f_1(\vx), \ldots, f_M(\vx)\right)}_\text{diversity regularizer}
        \! \Bigr]
    \end{split}
    \label{eqn:loss_gamma}
\end{equation}
%
where $\gamma$ is a hyperparameter (negative values encourage diversity; positive values discourage diversity) and $\mathbb{D}$ is some measure of predictive diversity.
%
\begin{enumerate}[leftmargin=*,topsep=0pt]
\item {\bf Variance} regularization \citep{ortega2022diversity} sets $\mathbb D$ to:
    \[
        \mathbb{E}_{p(\vx,y)}\left[
            \tfrac{1}{2(M-1) \max_{i}f_{i}^{y}(x)} \tsum_{i=1}^M
            \left(f_{i}^{y}(x) - \bar f_{i}^{y}(x)\right)^2
        \right],
    \]
    which essentially corresponds to the variance over ensemble members' true-class predictions.

\item {\bf 1-vs-All Jensen-Shannon Divergence}-based regularization \citep{mishtal2012jensen} sets $\mathbb D$ to:
    \[
        \mathbb{E}_{p(\vx,y)}\left[\tfrac{1}{M}\tsum_{i=1}^M JS \left(
            \vf_i(x) \:\middle\Vert\: \tfrac{1}{M-1}\tsum_{j\neq i}\vf_j(x)
        \right) \right],
    \]
    where $\text{JS}$ is the Jensen-Shannon divergence.

\item {\bf Uniform Jensen-Shannon Divergence}-based regularization \citep{zhao2022towards} sets $\mathbb D$ to:
    \begin{equation}
        \mathbb{E}_{p(\vx)}\left[
            H\left( \bar\vf(\vx) \right) -
            \tfrac{1}{M}\tsum_{i=1}^M H\left(\vf_i(\vx)\right),
        \right]
        \nonumber
    \end{equation}
    where $H$ is Shannon entropy.
    Note that the term inside the brackets is equivalent to the multi-distribution Jensen-Shannon divergence with uniform weights.
\item {\bf {Jensen Gap}}-based regularization (as introduced in \citep{abe2022the}).
Finally, closely corresponding to the Jensen gap analysis in \cref{sec:measuring_diversity}, we consider the following objective function to encourage/discourage diversity: 
\begin{equation}
\E_{p(\vx, y)} \Bigl[ \:
        \ell \left( \bar \vf(\vx), y \right) 
    +
        (\gamma+1) \left( \tfrac 1 M \tsum_{i=1}^M \ell \left( \vf_i(\vx), y \right)- \ell \left( \bar \vf(\vx), y \right) \right)
\: \Bigr].
\nonumber
\end{equation}

The first term is the risk associated with ensemble predictions (as opposed to the average single model risk),
while the second term is the Jensen gap notion of predictive diversity. .
\end{enumerate}

For all methods, $\gamma=0$ corresponds to standard ensemble training, setting $\gamma < 0$ encourages a more diversity, and setting $\gamma > 0$ discourages diversity.

The first two methods were designed to encourage ensemble diversity \citep{ortega2022diversity,mishtal2012jensen}, while the third was originally used as a regularizer for large-model training \citep{zhao2022towards}. The forth has previously been applied to encourage and discourage predictive diversity, but only for a handful of models.
In these experiments, we go beyond their original uses by both encouraging and discouraging predictive diversity across many architectures and tasks.

Note that we will not compare performance across the different regularizers, but instead focus on whether encouraging or discouraging follows the same trends throughout. 

Beyond the diversity regularizers above, 
we omit experiments with bagging, as its detrimental effects on deep ensembles are well established \citep{Nixon2020-hw}. Moreover, bagging can only be used to encourage diversity; it cannot be reformulated to discourage diversity.
Finally, we do not consider boosting, as this method is designed for weak learners.


\textbf{Datasets and Architectures}.
We train deep ensembles on the CIFAR10, CIFAR100  \citep{krizhevsky2009learning} TinyImageNet \citep{le2015tiny} and ImageNet \citep{deng2009imagenet} datasets.
Ensembles consist of $M=4$ models of the same neural network architecture for all datasets except ImageNet, where $M=3$.
We construct ensembles using both high and low capacity architectures, which we differentiate based on their ability to achieve perfect accuracy on the training dataset.
The high capacity architectures we consider for the CIFAR datasets are: ResNet 18 \citep{he2016deep}, VGG 11 \citep{simonyan2014very}, WideResNet 28-10 \citep{zagoruyko2016wide}, and DenseNet 121 (DenseNet 161 for CIFAR100) \citep{huang2017densely}. We additionally train ResNet 34 models on the TinyImageNet dataset, and ResNet18 on ImageNet. 
The low capacity architectures we consider are ResNet 8 and LeNet \citep{lecun1998gradient}.
See \cref{appx:modeltraining} for training and implementation details.

\textbf{Classes of ensembles.} We  
contrast the behavior of \emph{(high-capacity classification) deep ensembles} with regression deep ensembles and low-capacity deep ensembles. 

\textit{Ensembles of regression neural networks.}
We apply regression ensembles to CIFAR10/CIFAR100 by framing classification as regression \cite{hui2020evaluation,demirkaya2020exploring}.
In this setting the model outputs are not required to add up to 1 (i.e. the prediction space is unconstrained),
so Observation 2 does not apply to these ensembles.
Consequentially, we hypothesize that diversity encouragement will not harm performance.
For these models, $\ell$ is mean squared error and we study only the Jensen Gap regularizer, which corresponds to regularizing variance (see \cref{appx:variance_decomposition}). In this setting, the other regularizers above become redundant with Jensen Gap, or do not apply, as they are specific to classification settings. 

\begin{wrapfigure}{R}{0.40\textwidth}
\vspace{-2em}
\centering
\subfloat{\includegraphics[width=\linewidth]{figs/casr_cifar10_wideresnet28_10.pdf}}
\vspace{-0.5em}
\caption{\textbf{With MSE loss, encouraging predictive diversity does not hurt performance}. We also train deep regression ensembles using  \cref{eqn:ens_training_objective} with to MSE loss, on CIFAR10 and CIFAR100 (coarse lables). As predicted by our hypothesis, encouraging diversity does not hurt predictive performance in regression.
}
\label{fig:classification_as_regression}
\vspace{-2em}
\end{wrapfigure}

\textit{Ensembles of low-capacity classification neural networks.} Finally, we study ensembles of small classification models.
To the best of our knowledge, low-capacity models are the only setting where previous literature has demonstrated the benefits of diversity encouragement \cite{mishtal2012jensen,webb2020ensemble,ortega2022diversity}. These models make predictions with lower confidence than modern deep ensembles \citep{guo2017calibration}, so we hypothesize that most predictions will not approach the boundaries of the prediction space (see Observation 2), thus avoiding the pathological behavior we hypothesize for large-model classification ensembles. For these ensembles---as well as the high-capacity ensembles---$\ell$ is the cross entropy loss.  



\begin{figure*}[!t]
\centering
\subfloat{\includegraphics[width=\linewidth]{figs/all_weight_resnet8_cifar10.pdf}}
\vspace{-1em}
\caption{\textbf{Diversity encouragement helps performance for low-capacity models.} Low capacity ensembles are trained on CIFAR10 using the loss in \cref{eqn:loss_gamma} (for CIFAR100 and another architecture, see \cref{appx:replications}). For low-capacity models, diversity encouragement with the same regularizers and datasets shown in \cref{fig:diversity_plots} can produce improved performance, and discouraging diversity hurts performance. This result is consistent with our hypothesis that the effect of diversity encouragement depends on the magnitude of ensemble predictions (and thus the confidence of ensemble predictions). 
}
\vspace{-1em}
\label{fig:underparam_diversity}
\end{figure*}



\subsection{Diversity Regularization Results}

Across different architectures, datasets, and diversity regularizations, we find large classification ensembles exhibit drastically different behavior from other ensemble types.  


\textbf{Encouraging diversity harms test performance in large scale models.}
In \cref{fig:diversity_plots}, we illustrate the performance of diversity regularized ensembles of ResNet18 networks for CIFAR10.
(See \cref{appx:replications} for VGG, WideResNet, and DenseNet ensembles, as well as results on CIFAR100, TinyImageNet and ImageNet). 
In \cref{fig:diversity_plots}, the blue line and bands depict standard (unregularized) ensemble performance (mean $\pm$ two standard error).  
The black line and bands depict the error of single models.
Against these baselines, each panel of \cref{fig:diversity_plots} shows the performance of individual ensembles trained with different regularizers and values of $\gamma$. 
Across all diversity regularizers and datasets, ensembles with a downweighted diversity penalty ($\gamma < 0$) have \textit{much worse performance} than the ensemble trained with unmodified objective ($\gamma=0$). 
In some cases, the performance undershoots that of a single network.


In \cref{appx:metrics_diversity_regularization}, we show that the performance of these ensembles on probabilistic performance metrics (NLL, Brier Score, and ECE) also follow the same trends. 

In \cref{fig:biasvar_decomp}, 
we decompose the performance of these ensembles into predictive diversity (x axis), and average single model performance (y axis) (see Eq.~\ref{eqn:tradeoffs}). Relative to standard ensemble training (indicated with $\times$), we see that ensembles trained with diversity-encouragement (blue dots) indeed express more predictive diversity. However, we see that this increase comes at the cost of single model performance, mirroring the anticorrelation between predictive diversity and single model performance observed in \cref{fig:all_indep_models}. The overall effect of encouraging predictive diversity is higher values of the ensemble loss (level sets further up and to the left). 



\textbf{Discouraging predictive diversity can be beneficial to predictive performance. 
}
In contrast, \cref{fig:diversity_plots} shows that further penalizing diversity (i.e. $\gamma > 0$ in the Jensen Gap plots) also behaves unexpectedly.
(Again, see \cref{appx:replications} for CIFAR100 results, as well as VGG, Wide ResNet, and DenseNet ensembles.)
In most cases diversity discouragement leaves predictive performance intact, across the range of studied regularization strength.
Overall in $56\%$ of the 149 experiments where diversity was discouraged, performance remains intact, while it decreases in $28\%$, and even improves for $20\%$ of the ensembles (\cref{table:summary_discourage}).

In \cref{fig:biasvar_decomp}, we once again use the decomposition offered by \cref{eqn:tradeoffs} to analyze the effect of diversity-discouragement.
We note that in many cases, discouraging diversity leads to ensembles with improved average single model performance.
In all cases, the best performing ensembles (lowest level set) are trained with diversity discouragement. 
 


\textbf{Encouraging diversity does not hurt regression ensembles.}
\cref{fig:classification_as_regression} demonstrates that diversity encouragement exhibits markedly different trends for regression ensembles.
We plot the predictive performance of a WideResNet28-10 ensemble (trained with the MSE loss rather than cross-entropy) trained with diversity encouragement/discouragement.  (See \cref{appx:replications} for DenseNet ensembles.)
Unlike in \cref{fig:diversity_plots}, the majority of ensembles trained with diversity encouragement (12/16) improve upon baseline performance, with improvements proportional to regularization strength.  
In contrast, the effect of discouraging predictive diversity appears to be dataset specific, leading to uniformly worse performance on CIFAR10 data, but leading to consistent improvements on CIFAR100, as in the case with large-model classification ensembles.

\textbf{Encouraging diversity does not hurt low capacity models.} Finally, \cref{fig:underparam_diversity} demonstrates that low-capacity classification ensembles exhibit the \emph{opposite} behavior of their large-capacity counterparts.
We repeat the experiment in \cref{fig:diversity_plots} for the smaller ResNet 8 architecture on CIFAR10.
(See \cref{appx:replications} for CIFAR100 and LeNet ensembles.)
Relative to the standard ensemble baseline (blue band), each regularizer has at least one range of values where encouraging diversity leads to performance improvements  ensembles, and discouraging diversity appears to yield consistently worse performance.
In total, diversity encouragement improves the performance of $73\%$ of 86 low capacity ensembles. 


Here we note that the distinction between low-capacity and high-capacity models also appears to govern the trade-off between predictive diversity and average single model performance in models trained without diversity regularization. Returning to \cref{fig:all_indep_models} we see that the anticorrelation between average single model performance and diversity only appears when we consider models that achieve a certain level of performance, and are thus presumably of large capacity. 
Notably, in \cref{table:imagenet}, we show that encouraging predictive diversity for ResNet18 ensembles fails even on the very large ImageNet dataset. We hypothesize that this is because models that are technically underparametrized relative to a dataset still make a significant proportion of their predictions with high confidence \cref{appx:imagenet}, leaving them susceptible to Observation 2 . 
\cref{table:summary,table:summary_discourage} in \cref{appx:replications} summarize our results.


\textbf{Additional results}.  
In \cref{appx:diversity_regularization_other} we apply the ensembles from \cref{fig:diversity_plots} to CIFAR10.1 \citep{recht2018cifar}, an out of distribution (OOD) test dataset for CIFAR10. 
Our results show that encouraging diversity during training poses no benefits over standard deep ensembles.


In \cref{appx:other_hypothesistests}, we examine the effects of diversity encouragement/discouragement on ensembles trained with a label smoothing loss \citep{szegedy2016rethinking}.
The targets for label smoothing are located away from the probability simplex vertices, which makes it possible to maintain accuracy while achieving some level of predictive diversity.
Our results suggest label smoothing 
could ameliorate the harmful effects of diversity encouragement, but it does not change the overall trend in \cref{fig:diversity_plots}. 


==> sections/intuition.tex <==
\begin{wrapfigure}{L}{0.3\textwidth}
    % \centering
    \includegraphics[width=0.9\linewidth]{figs/update_div_3.pdf}
    \vspace{-0.5em}
    \caption{
        \textbf{For classification tasks, encouraging diversity during training worsens confident/accurate predictions.}
        With probabilistic predictions, outputs of individual ensemble members ($\times$) lie in a simplex. 
        The ensemble prediction (circle) is the average of these predictions. 
        If ensemble outputs are highly confident and accurate (top panel), more diversity (left) necessarily degrades the confidence of the ensemble prediction, or results in errors. In contrast, less diversity (right) need not hurt ensemble predictions.
    }
    \label{fig:diversity_intuition}
    \vspace{-2em}
\end{wrapfigure}
\section{Rethinking predictive diversity for deep ensembles}
\label{sec:intuition}

% In standard deep ensembling, predictive diversity in \cref{eqn:tradeoffs} is due only to random initialization and training of ensemble members. 
% We define \textit{diversity interventions} as alterations of existing ensemble methods which aim to increase predictive diversity between ensemble members. 
% Intuitively, a diversity intervention which does not degrade $\mathcal{L}_{avg}$ would improve ensemble performance (\cref{fig:schematic}, rightwards arrow). 
However, in this section we argue that any diversity intervention will negatively influence ensembles which already make accurate, confident predictions, with the prime example being deep ensembles. 

\textbf{Diversity interventions impact correct predictions as well as errors.}
The motivation for diversity interventions is decorrelation of predictions where the ensemble would have otherwise made an error  \citep[e.g.][]{liu1999ensemble,dietterich2000ensemble,mishtal2012jensen,ortega2022diversity}, thereby improving ensemble performance. 
% Error decorrelation is presented as the primary function of diversity mechanisms, and the source of their benefits. 
Inevitably however, diversity interventions will also influence predictions where the ensemble would have otherwise been correct (as they would otherwise be oracle error detectors). 
As we form ensembles from increasingly accurate models, we would expect that decorrelation of correct predictions becomes an increasingly significant consequence of any diversity intervention. 
We provide experimental evidence for this claim in \cref{appx:counterfactual}, where we consider ensembles of trees (with random forests as the diversity mechanism) and ResNet 18 neural networks (with the Jensen Gap and Variance regularizers as a diversity mechanism- see \cref{sec:experimental_setup} for details). 
In both, we see that interventions which encourage greater levels of predictive diversity do so by decorrelating a greater proportion of accurate, confident predictions.

% 
% We plot the \textit{counterfactual accuracy} of an ensemble (in the absence of diversity encouragement) as a function of the diversity encouraged at individual test points. For both trees (with random forests as the diversity mechanism) and deep ensembles (with the Jensen Gap as a diversity mechanism- see \cref{sec:experimental_setup}), we see that 
% We confirm the effect of diversity regularization on these counterfactually correct predictions in Figure \cref{fig:todo}. 



\textbf{Risk of diversifying correct predictions increases with model scale.}
In some cases, increasing predictive diversity could leave a correct prediction unchanged: even if ensemble members make more diverse predictions, they could potentially``average out'', leaving the ensemble prediction unaffected. 
However, this assumption breaks down in the case where we are ensembling large, powerful classification models.
Since large classification neural networks tend to be extremely confident \citep{guo2017calibration}, component model predictions will all concentrate in the same vertex of the probability simplex (see \cref{fig:diversity_intuition}, ``Standard Ensembling'').
In this case, it is impossible to increase predictive diversity without harming the ensemble loss in \cref{eqn:tradeoffs}. 
Increasing diversity would necessarily require at least one component model to become less confident, which could not be counteracted by other models since their predictions already lie on an extreme point of the simplex.
As a consequence, encouraging diversity would necessarily cause the average prediction to become less confident, and may potentially move across the decision boundary (see \cref{fig:diversity_intuition}, ``Diversity Encouraged'').
We note that this is not an issue for regression---since predictions are unconstrained---nor for small-model classification---since predictions are less confident and thus lie in a portion of the simplex that can be locally approximated by an unbounded space.
% However, we have reason to expect that these issues should generalize to large datasets lie ImageNet \citep{deng2009imagenet}, given that commonly used models are already making accurate predictions on such datasets with high confidence \cref{appx:imagenet}. 


% In some cases, diversifying counterfactually correct predictions could leave ensemble performance unchanged. 

% From \cref{fig:all_indep_models} we see that predictive diversity contributes less to the performance of deep ensembles for classification tasks than to other ensembles (e.g. formed from decision trees). 
% Although it is tempting to view this discrepancy as an opportunity for improvement, we identify two features of large classification models which preclude any benefits of diversity encouragement. 

% What would happen if we were to encourage additional predictive diversity by modifying the ensemble training objective in \cref{eqn:ens_training_objective}?
% Though a direct intervention may be beneficial in certain ensembling scenarios \citep[e.g.][]{mishtal2012jensen,webb2020ensemble,ortega2022diversity},
% we do not expect the same benefits for the deep ensembles we are concerned with.
% This hypothesis is based on two observations about large classification models---%
% which we empirically confirm in \cref{sec:analysis}:


% \textbf{Observation 1: Encouraging diversity during training affects all predictions, not only errors.}
% The mechanism by which encouraging diversity improves ensembling can be understood counterfactually.
% If ensemble members all make the same error on a test datapoint, diversity encouragement creates an ensemble where some classifiers instead make different errors, or even find the correct solution, thereby improving both terms on the left hand of \cref{eqn:tradeoffs}. 
% In contrast however, if ensemble members all agree on the same correct solution, diversity encouragement has the potential to harm this prediction, increasing average single model loss even as predictive diversity is increased. Therefore, all methods for diversity encouragement implicitly rely on the idea that erroneous test points will be influenced more strongly than those where ensemble members are already correct. 

% % In an ideal world, it would be possible to increase the predictive diversity around erroneous model predictions (i.e. decorrelating errors)
% % while leaving otherwise correct predictions untouched.
% % However, it is highly unlikely that any training intervention could selectively increase predictive diversity in such a way.
% However, recent evidence suggests that both correct and erroneous predictions made by modern neural networks are driven by robust inductive biases.
% \citet{feldman2020neural,feldman2020does} demonstrate the role of 
% data memorization in the performance of large scale neural networks, and \citet{abe2022deep} show that the predictions of a large neural network is highly correlated with an ensemble of smaller networks with similar performance. Strikingly, \citet{mania2019model,mania2020classifier,geirhos2020beyond} demonstrate that neural network classifiers make correlated errors, even across different architectures. 
% When errors are largely driven by inductive bias, diversity encouragement should be just as likely to decorrelate accurate and confident predictions (which already constitute a much larger portion of the test set) as often as they do errors. Indeed, we empirically demonstrate this finding in \cref{sec:analysis}. 

% \textbf{Observation 2: In constrained prediction spaces, diversity is impossible at extreme points.}
% Intuitively, one of the major benefits of ensembling is the possibility that the ensemble prediction may be correct, even when no individual ensemble member is correct. 

% In the case of classification, the impact of diversity encouragement on otherwise correct predictions is magnified. 
% % With Observation 1 in mind, we demonstrate why increasing diversity for otherwise accurate predictions is potentially harmful.
% Since large classification neural networks tend to be extremely confident \citep{guo2017calibration}, component model predictions will all concentrate in the same vertex of the probability simplex (see \cref{fig:diversity_intuition}, ``Standard Ensembling'').
% In this case, it is impossible to increase predictive diversity without harming the ensemble loss in \cref{eqn:tradeoffs}. 
% Increasing diversity would necessarily require at least one component model to become less confident, which could not be counteracted by other models since their predictions already lie on an extreme point of the simplex.
% As a consequence, encouraging diversity would necessarily cause the average prediction to become less confident, and may potentially move across the decision boundary (see \cref{fig:diversity_intuition}, ``Diversity Encouraged'').
% We note that this is not an issue for regression---since predictions are unconstrained---nor for small-model classification---since predictions are less confident and thus lie in a portion of the simplex that can be locally approximated by an unbounded space. However, we have reason to expect that these issues should generalize to large datasets lie ImageNet \citep{deng2009imagenet}, given that commonly used models are already making accurate predictions on such datasets with high confidence \cref{appx:imagenet}. 



\textbf{Discouraging predictive diversity.}
Given intuitions from the existing ensemble literature, it would be natural to assume that discouraging predictive diversity should harm performance.
Taken to an extreme, discouraging diversity would result in all component models producing the same prediction, removing any benefits of ensembling.
However, our understanding from the previous observations paint a different picture.
% If many of the errors made by ensemble members are already highly correlated (as suggested by Observation 1), we would expect few performance deficits from further correlating these errors.
% Moreover, there is reason to expect that discouraging diversity could potentially be beneficial.
Recent theoretical evidence suggests that increasing the capacity of overparameterized models amounts to variance reduction \cite{neal2018modern,adlam2020understanding}---a result which is further supported empirically by \cref{fig:all_indep_models}, and other work on ensemble distillation \citep{zhu2018knowledge,zhao2022towards}.
Discouraging diversity through the use of a regularizer is an alternative path towards variance reduction that could mimic the effects of larger models.


==> tables/extra_mean_cifar10_resnet18.tex <==
\begin{tabular}{lllllllll}
\toprule
          Diversity (Jensen Gap) & Stat. &  &     No Regularizer &  &          Jensen Gap &            Variance &        JSD 1-vs-All &         JSD Uniform \\
\midrule
\midrule
(0.024, 0.1] & Baseline Ens. CE &          &  $0.787 \pm 0.050$ &          &   $0.740 \pm 0.024$ &   $0.639 \pm 0.024$ &   $0.170 \pm 0.003$ &   $0.210 \pm 0.005$ \\
           & $p$ @ $5\%$ Increase &          &                --- &          &             $0.117$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
           & $p$ @ $25\%$ Increase &          &                --- &          &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
\midrule
(0.1, 0.25] & Baseline Ens. CE &          &  $1.107 \pm 0.055$ &          &   $0.998 \pm 0.027$ &   $0.153 \pm 0.002$ &   $0.290 \pm 0.006$ &   $0.883 \pm 0.023$ \\
           & $p$ @ $5\%$ Increase &          &                --- &          &  $\mathbf{ 0.010 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
           & $p$ @ $25\%$ Increase &          &                --- &          &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
\midrule
(0.25, 0.5] & Baseline Ens. CE &          &  $1.293 \pm 0.047$ &          &   $0.217 \pm 0.004$ &   $0.519 \pm 0.011$ &   $0.872 \pm 0.016$ &   $1.041 \pm 0.022$ \\
           & $p$ @ $5\%$ Increase &          &                --- &          &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
           & $p$ @ $25\%$ Increase &          &                --- &          &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
\midrule
(0.5, 1.0] & Baseline Ens. CE &          &  $1.411 \pm 0.043$ &          &   $0.490 \pm 0.008$ &   $0.415 \pm 0.008$ &   $1.125 \pm 0.017$ &   $1.263 \pm 0.023$ \\
           & $p$ @ $5\%$ Increase &          &                --- &          &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
           & $p$ @ $25\%$ Increase &          &                --- &          &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.000 }$ \\
\midrule
(1.0, $\infty$] & Baseline Ens. CE &          &  $1.505 \pm 0.064$ &          &   $1.241 \pm 0.024$ &   $1.458 \pm 0.044$ &   $1.727 \pm 0.027$ &   $1.820 \pm 0.051$ \\
           & $p$ @ $5\%$ Increase &          &                --- &          &  $\mathbf{ 0.027 }$ &             $0.476$ &             $1.000$ &             $1.000$ \\
           & $p$ @ $25\%$ Increase &          &                --- &          &  $\mathbf{ 0.000 }$ &  $\mathbf{ 0.014 }$ &             $0.326$ &             $0.694$ \\
\bottomrule
\end{tabular}

==> tables/results_summary.tex <==
\begin{table}[H]
\begin{center}
\resizebox{0.4\linewidth}{!}{%
    \begin{tabular}{|| m{9.1em} |  m{3em} | m{3em} | m{3em} ||} 
      \hline
     Diversity Encouragement... & Hurts & Neutral & Helps \\
     \hline\hline
     Small NN Classification Ensembles & 12/85 ($14\%$) & 7/85 ($8\%$) & 66/85 ($78\%$) \\
     \hline
     NN Regression Ensembles & 3/16 ($19\%$) & 1/16 ($6\%$) & 12/16 ($75\%$) \\
     \hline
     Large overconfident NN Classification Ensembles & 82/134 ($61\%$) & 38/134 ($29\%$) & 14/134 ($10\%$) \\
     \hline
    \end{tabular}
}
\caption{\textbf{Modern Deep Ensembles Respond Differently to Diversity Encouragement}. Across a large number of experimental settings, we see that encouraging predictive diversity has opposite effects on modern deep ensembles (Large Overconfident Classification Ensembles) vs. other types of ensembles. The classification of ensembles listed is calculated relative to 2 standard error of single ensemble performance.}
\label{table:summary}
\end{center}
\end{table}

\begin{table}[H]
\begin{center}
\resizebox{0.4\linewidth}{!}{%
    \begin{tabular}{|| m{9.1em} |  m{3em} | m{3em} | m{3em} ||} 
      \hline
     Diversity Discouragement... & Hurts & Neutral & Helps \\
     \hline\hline
     Small NN Classification Ensembles & 46/82 ($56\%$) & 33/82 ($40\%$) & 3/82 ($4\%$) \\
     \hline
     NN Regression Ensembles & 8/13 ($62\%$) & 1/13 ($8\%$) & 4/13 ($3\%$) \\
     \hline
     Large Overconfident NN Classification Ensembles & 41/156 ($26\%$) & 78/156 ($50\%$) & 37/156 ($24\%$) \\
     \hline
    \end{tabular}
}
\caption{\textbf{Modern Deep Ensembles Respond Differently to Diversity Discouragement}. Across a large number of experimental settings, we see that discouraging predictive diversity has opposite effects on modern deep ensembles (Large Overconfident Classification Ensembles) vs. other types of ensembles. The classification of ensembles listed is calculated relative to 2 standard error of single ensemble performance.}
\label{table:summary_discourage}
\end{center}
\end{table}
